MST-compression: Compressing and Accelerating Binary Neural Networks with Minimum Spanning Tree

Binary neural networks (BNNs) have been widely adopted to reduce the computational cost and memory storage on edge-computing devices by using one-bit representation for activations and weights. However, as neural networks become wider/deeper to improve accuracy and meet practical requirements, the computational burden remains a significant challenge even on the binary version. To address these issues, this paper proposes a novel method called Minimum Spanning Tree (MST) compression that learns to compress and accelerate BNNs. The proposed architecture leverages an observation from previous works that an output channel in a binary convolution can be computed using another output channel and XNOR operations with weights that differ from the weights of the reused channel. We first construct a fully connected graph with vertices corresponding to output channels, where the distance between two vertices is the number of different values between the weight sets used for these outputs. Then, the MST of the graph with the minimum depth is proposed to reorder output calculations, aiming to reduce computational cost and latency. Moreover, we propose a new learning algorithm to reduce the total MST distance during training. Experimental results on benchmark models demonstrate that our method achieves significant compression ratios with negligible accuracy drops, making it a promising approach for resource-constrained edge-computing devices.

==> TIKZ/data-loss/train_error.tex <==
5	86.584
10	88.306
15	88.276
20	88.654
25	88.468
30	88.838
35	88.406
40	88.456
45	88.532
50	88.392
55	88.6
60	88.56
65	88.542
70	88.426
75	88.318
80	88.556
85	88.32
90	88.372
95	88.41
100	88.488
105	88.396
110	88.23
115	88.588
120	88.56
125	88.508
130	88.58
135	88.518
140	88.45
145	88.134
150	88.67
155	88.524
160	88.81
165	88.782
170	88.822
175	89.028
180	88.982
185	88.982
190	89.168
195	88.974
200	89.15
205	89.428
210	89.466
215	89.424
220	89.646
225	89.748
230	89.632
235	89.642
240	89.864
245	89.988
250	89.99
255	89.902
260	90.21
265	90.212
270	90.402
275	90.35
280	90.562
285	90.462
290	90.854
295	90.734
300	90.83
305	91.196
310	91.088
315	91.25
320	91.278
325	91.548
330	91.672
335	91.636
340	91.848
345	92.3
350	92.108
355	92.196
360	92.658
365	92.784
370	92.972
375	93.064
380	93.354
385	93.348
390	93.518
395	93.698
400	93.942
405	94.062
410	94.358
415	94.352
420	94.534
425	94.658
430	94.878
435	95.134
440	95.316
445	95.552
450	95.524
455	95.81
460	96.114
465	96.274
470	96.372
475	96.614
480	96.714
485	97.016
490	97.218
495	97.254
500	97.494
505	97.632
510	97.636
515	98.024
520	97.96
525	98.106
530	98.254
535	98.41
540	98.55
545	98.542
550	98.738
555	98.824
560	98.974
565	99.034
570	99.132
575	99.094
580	99.156
585	99.228
590	99.284
595	99.276
600	99.198


==> TIKZ/data-loss/val_error.tex <==
5	41.29
10	68.4
15	42.96
20	53.83
25	28.64
30	51.21
35	57.84
40	68.21
45	40.38
50	52.13
55	40.8
60	40.85
65	63.91
70	53.67
75	52.01
80	65.25
85	66.43
90	73.84
95	68.17
100	40.88
105	51.23
110	20.35
115	37.39
120	70.03
125	70.07
130	63.61
135	67.71
140	22.35
145	54.87
150	69.73
155	55.76
160	50.45
165	52.72
170	56.94
175	44.08
180	76.5
185	58.83
190	61.88
195	73.88
200	78.09
205	54.42
210	66.7
215	66.11
220	63.98
225	71.75
230	62.38
235	76.64
240	72.69
245	71.88
250	70.43
255	74.01
260	66.54
265	80.36
270	72.25
275	69.22
280	63.14
285	68.79
290	68.6
295	68.82
300	68.71
305	69.12
310	79.25
315	55.26
320	77.21
325	83.66
330	77.72
335	68.46
340	78.72
345	73.48
350	78.88
355	75.21
360	82.63
365	75.62
370	77.72
375	81.47
380	81.55
385	83.95
390	82.02
395	80.18
400	73.36
405	83.74
410	73.19
415	83
420	78.71
425	86.25
430	77.87
435	77.08
440	85.45
445	80.28
450	76.11
455	84.68
460	81.36
465	83.52
470	81.61
475	75.5
480	75.81
485	85.37
490	84.32
495	83.57
500	79.82
505	86.91
510	86.52
515	83.99
520	83.05
525	83.25
530	87.57
535	89.43
540	88.14
545	85.03
550	87.08
555	88.85
560	89.88
565	90.01
570	90.4
575	88.98
580	91.15
585	90.56
590	90.92
595	91.29
600	91.12


==> TIKZ/tikz_styles.tex <==
\usepackage{pgfplots}

\pgfplotsset{
	curve plot style/.style={
		xlabel={X-axis description},
		xmin=0, xmax=600,
		%xtick={1,2,3,4,5,6},
		ytick={300000,50000,80000,100000,150000,200000,250000,300000,350000},
		legend pos=north east,
		ymajorgrids=true,     xmajorgrids=true,
		grid style=dashed,
		ylabel={Y-axis description},
		ylabel style={yshift=-.5cm},
		width=8.5cm,
		height=10cm,
	},
}




